RikoNet: A Novel Anime Recommendation Engine

Anime is quite well-received today, especially among the younger generations. With many genres of available shows, more and more people are increasingly getting attracted to this niche section of the entertainment industry. As anime has recently garnered mainstream attention, we have insufficient information regarding users' penchant and watching habits. Therefore, it is an uphill task to build a recommendation engine for this relatively obscure entertainment medium. In this attempt, we have built a novel hybrid recommendation system that could act both as a recommendation system and as a means of exploring new anime genres and titles. We have analyzed the general trends in this field and the users' watching habits for coming up with our efficacious solution. Our solution employs deep autoencoders for the tasks of predicting ratings and generating embeddings. Following this, we formed clusters using the embeddings of the anime titles. These clusters form the search space for anime with similarities and are used to find anime similar to the ones liked and disliked by the user. This method, combined with the predicted ratings, forms the novel hybrid filter. In this article, we have demonstrated this idea and compared the performance of our implemented model with the existing state-of-the-art techniques.

==> Recommendation System Paper/new_related_work.tex <==
[10]	Vie, Jill-Jenn & Yger, Florian & Lahfa, Ryan & Clement, Basile & Cocchi, Kevin & Chalumeau, Thomas & Kashima, Hisashi. (2017). Using Posters to Recommend Anime and Mangas in a Cold-Start Scenario. 21-26. 10.1109/ICDAR.2017.287.

[11]	Syoichiro Ota, Hayaki Kawata, Masahumi Muta, Soh Masuko, Jun’ichi Hoshino. AniReco: Japanese Anime Recommendation System. 16th International Conference on Entertainment Computing (ICEC), Sep 2017, Tsukuba City, Japan. pp.400-403, 10.1007/978-3-319-66715-7$_$49. hal-01771283
[12]	Mohan, Geetha & Iqubal, Safa & Fancy, C & Saranya, D. (2018). A Hybrid Approach using Collaborative filtering and Content based Filtering for Recommender System. Journal of Physics: Conference Series. 1000. 012101. 10.1088/1742-6596/1000/1/012101.
[13]	Putri, Debby & Leu, Jenq-Shiou & Seda, Pavel. (2020). Design of an Unsupervised Machine Learning-Based Movie Recommender System. Symmetry. 12. 185. 10.3390/sym12020185.

[14]	Hyun-Tae Kim, Jong-Hyun Lee, Chang Wook Ahn, “A recommender system based on interactive evolutionary computation with data grouping”, Procedia Computer Science, Volume 3, 2011, Pages 611-616, ISSN 1877-0509
[15]	Girsang, A & Al Faruq, Barra & Herlianto, Hemdani & Simbolon, Sihar. (2020). Collaborative Recommendation System in Users of Anime Films. Journal of Physics: Conference Series. 1566. 012057. 10.1088/1742-6596/1566/1/012057.
[16]	Amer Al-Badarenah, Jamal Alsakran, ―An Automated Recommender System for Course Selection‖, International Journal of Advanced Computer Science and Applications, Vol.7, No.3, pp. 166- 173, 2016.
[17]	Tengku Azfar, & Su-Cheng Haw. (2020). EVALUATION OF HYBRID RECOMMENDER TECHNIQUES ON MOVIELENS DATASET. PalArch’s Journal of Archaeology of Egypt / Egyptology, 17(10), 890-902. 

[18]	Nápoles, Gonzalo & Grau, Isel & Salgueiro, Yamisleydi. (2020). Recommender System using Long-term Cognitive Networks. Knowledge-Based Systems. 206. 10.1016/j.knosys.2020.106372.

[19]	Harpreet Kaur Virk, Er. Maninder Singh,” Analysis and Design of Hybrid Online Movie Recommender System ”International Journal of Innovations in Engineering and Technology (IJIET) Volume 5 Issue 2,April 2015.


==> new_related_work.tex <==
[10]	Vie, Jill-Jenn & Yger, Florian & Lahfa, Ryan & Clement, Basile & Cocchi, Kevin & Chalumeau, Thomas & Kashima, Hisashi. (2017). Using Posters to Recommend Anime and Mangas in a Cold-Start Scenario. 21-26. 10.1109/ICDAR.2017.287.

[11]	Syoichiro Ota, Hayaki Kawata, Masahumi Muta, Soh Masuko, Jun’ichi Hoshino. AniReco: Japanese Anime Recommendation System. 16th International Conference on Entertainment Computing (ICEC), Sep 2017, Tsukuba City, Japan. pp.400-403, 10.1007/978-3-319-66715-7$_$49. hal-01771283
[12]	Mohan, Geetha & Iqubal, Safa & Fancy, C & Saranya, D. (2018). A Hybrid Approach using Collaborative filtering and Content based Filtering for Recommender System. Journal of Physics: Conference Series. 1000. 012101. 10.1088/1742-6596/1000/1/012101.
[13]	Putri, Debby & Leu, Jenq-Shiou & Seda, Pavel. (2020). Design of an Unsupervised Machine Learning-Based Movie Recommender System. Symmetry. 12. 185. 10.3390/sym12020185.

[14]	Hyun-Tae Kim, Jong-Hyun Lee, Chang Wook Ahn, “A recommender system based on interactive evolutionary computation with data grouping”, Procedia Computer Science, Volume 3, 2011, Pages 611-616, ISSN 1877-0509
[15]	Girsang, A & Al Faruq, Barra & Herlianto, Hemdani & Simbolon, Sihar. (2020). Collaborative Recommendation System in Users of Anime Films. Journal of Physics: Conference Series. 1566. 012057. 10.1088/1742-6596/1566/1/012057.
[16]	Amer Al-Badarenah, Jamal Alsakran, ―An Automated Recommender System for Course Selection‖, International Journal of Advanced Computer Science and Applications, Vol.7, No.3, pp. 166- 173, 2016.
[17]	Tengku Azfar, & Su-Cheng Haw. (2020). EVALUATION OF HYBRID RECOMMENDER TECHNIQUES ON MOVIELENS DATASET. PalArch’s Journal of Archaeology of Egypt / Egyptology, 17(10), 890-902. 

[18]	Nápoles, Gonzalo & Grau, Isel & Salgueiro, Yamisleydi. (2020). Recommender System using Long-term Cognitive Networks. Knowledge-Based Systems. 206. 10.1016/j.knosys.2020.106372.

[19]	Harpreet Kaur Virk, Er. Maninder Singh,” Analysis and Design of Hybrid Online Movie Recommender System ”International Journal of Innovations in Engineering and Technology (IJIET) Volume 5 Issue 2,April 2015.

